Exact tensor completion using t-SVD

In this paper we focus on the problem of completion of multidimensional arrays (also referred to as tensors) from limited sampling. Our approach is based on a recently proposed tensor-Singular Value Decomposition (t-SVD) [1]. Using this factorization one can derive notion of tensor rank, referred to as the tensor tubal rank, which has optimality properties similar to that of matrix rank derived from SVD. As shown in [2] some multidimensional data, such as panning video sequences exhibit low tensor tubal rank and we look at the problem of completing such data under random sampling of the data cube. We show that by solving a convex optimization problem, which minimizes the tensor nuclear norm obtained as the convex relaxation of tensor tubal rank, one can guarantee recovery with overwhelming probability as long as samples in proportion to the degrees of freedom in t-SVD are observed. In this sense our results are order-wise optimal. The conditions under which this result holds are very similar to the incoherency conditions for the matrix completion, albeit we define incoherency under the algebraic set-up of t-SVD. We show the performance of the algorithm on some real data sets and compare it with other existing approaches based on tensor flattening and Tucker decomposition.

==> Literature_Survey.tex <==

\subsection{Related work}
\begin{figure*}
\begin{center}
\begin{tabular}{|l|c|c||r|}
\hline
  & reference & number of samples & incoherent condition \\ \hline
CP     & [1] & N/A & N/A \\ \hline
CP     & [5] & square deal:$Crn^{K/2}$ for CP rank $r$ & matrix case  \\ \hline
Tucker & [2] & N/A & N/A \\ \hline
Tucker & [5] & square deal:$Cr^{K/2}n^{K/2}$ for Tucker rank $(r,r,...,r)$ & matrix case \\ \hline
TSVD   & our paper & $Crnn_3 \log(nn_3)$ for 3rd-order tensor & our incoherent condition \\
\hline
\end{tabular}
\end{center}
\end{figure*}


\subsubsection{Tensor Completion based on CP format}

In [1], the authors try to complete a tensor which is low CP rank by solving the following optimization problem.

\begin{equation}
\min \|P_\Omega(\T{A} - \sum\limits_{\ell=1}^{L} x_\ell^{(1)} \circ x_\ell^{(2)} \circ ... \circ x_\ell^{(N)} ) \|^2_2 + \lambda \sum\limits_{\ell=1}^{L} \sum\limits_{n=1}^{N}\|x_\ell^{(n)}\|_2^2
\end{equation}
where $\lambda \ge 0$ is the regularization parameter. However, the complexity here which is summation of the $\ell_2$ norm of each tube is not a natural choice and lack of physical explanations. And due to the non-convexity of this problem, it only gaurantees local minimum. Also, there is no theoretic gaurantees of how many number of samples are actually required to recover the tensor exactly. Also, this method is hard to be used in practical problem since it is very hard to determine the CP rank of a tensor data beforehand, which is regarded as a prior in this approach.

\subsubsection{Tensor Completion based on Tucker Decomposition}

In[2], the authors focus on completing tensors which are supposed to be low rank in Tucker Decomposition. The problem they are dealing with is 

\begin{equation}
\begin{aligned}
\min_{X} \sum\limits_{i=1}^{n}\alpha_i \|\T{X}_i\|_*\\
\mbox{subject to  } \T{X}_{\Omega} = \T{T}_\Omega 
\end{aligned}
\end{equation}

For this method, there are no theoretical results on how to choose the weights $\alpha_i$ and basically one just choose the best dimension according to the results, which is in fact a matrix completion problem. 

There are some modified version of this case. [3] changes the complexity to the convex envelop of cardinality function of singular value vectors, which is proved to be a tighter convex relaxation of the Tucker rank comparing to the above approach. However, there is still no theoretical guarantees of number of samples needed in such cases.

Another paper [4], they are trying to solve the strong convex model:
\begin{equation}
\begin{aligned}
\min_{\T{X}} \sum\limits_{i=1}^{K}\lambda_i \|\T{X}_{i}\|_* + K \tau \|\T{X}\|^2_F \\
\mbox{subject to  } P_\Omega(\T{X}) = P_\Omega(\T{X}_0)
\end{aligned}
\end{equation}

It is claimed that if the above approach satisfies the Tensor Incoherent Condition(TIC), which is a direct extension of the matrix completion case, then a certain number(similar to matrix case) of samples are need for exact recovery. However, it is still not clear which unfolding is the best and the TIC here is very hard to satisfy for a large multi-dimension tensor.

[5] is another tensor completion problem. The authors are trying to complete a tensor which is supposed to be low-rank in Tucker Decomposition manner from Gaussian measurements. And certain optimality conditions are given. The idea is to reshape a multi-dimensional tensor $\T{X} \in \mathbb{R}^{n_1 \times n_2 \times n_3 \times ... \times n_K}$ into a matrix $\T{X}_{(j)} \in \mathbb{R}^{n_1 ... n_j \times n_{j+1}...n_{K}}$ and apply matrix completion on it. It can be shown easily that if $\T{X}_{(j)}$ is a low-rank tensor (in either CP or Tucker sense), $\T{X}_{(j)}$ will be a low-rank matrix. [5] claims that if $\T{X}_0$ has CP rank $r$, then $m \ge Crn^{K/2}$ will be sufficient. If $\T{X}_0$ has Tucker rank $(r,r,...,r)$, then $m \ge Cr^{K/2}n^{K/2}$ is sufficient. 


We note the following points. 
\begin{itemize}
\item If a tensor $\T{X}$ is low rank in Tucker and CP formats then it is also low t-SVD rank with t-SVD rank bounded by the Tucker or CP rank.
\item Further given an $[n_1,n_2,...,n_K]$ tensor one can reshape it to form a 3-D tensor of size $[n_1n_2..n_{k_1}, n_{k_1+1}..n_{K-1}, n_K]$ be \emph{reshaping} and then use our framework for 3-D tensor completion. If $n_k = n$ for all $k$ then it follows from our main results that ${\cal O}(n^{K/2} r^{K/2-1} n)$ measurements are sufficient enough for recovery.
\end{itemize}





\subsubsection{Reference}
\textbf{1} "Parallel Algorithms for Tensor Completion in the CP Format", Lars Karlsson, Daniel Kressner, Andr´e Uschmajew

\textbf{2} "Tensor Completion for Estimating Missing Values in Visual Data", Ji Liu, Przemyslaw Musialski, Peter Wonka, and Jieping Ye.

\textbf{3} "A New Convex Relaxation for Tensor Completion", Bernardino Romera-Paredes, Massimiliano Pontil.

\textbf{4} "LOW-RANK TENSOR RECOVERY: THEORY AND ALGORITHMS", Donald Goldfarb, Bo Huang, John Wright, Cun Mu,
Zhiwei Qin. availabel at \url{http://www.cerfacs.fr/algor/Recent_Advances_on_Optimization/Day_3/goldfarb.pdf}

\textbf{5} "Square Deal: Lower Bounds and Improved Relaxations for Tensor Recovery", Cun Mu, Bo Huang, John Wright, Donald Goldfarb1

\textbf{6} "Provable Low-Rank Tensor Recovery" \url{https://drive.google.com/viewerng/viewer?a=v&pid=sites&srcid=ZGVmYXVsdGRvbWFpbnxtdWN1bjE5ODh8Z3g6N2NlYjg1MGRkY2YxMTFjMQ}

\textbf{7} "Provable Tensor Factorization with Missing Data"
\url{http://papers.nips.cc/paper/5475-provable-tensor-factorization-with-missing-data.pdf}

\textbf{8} "Low-Rank Matrix and Tensor Completion via Adaptive
Sampling"

==> introduction.tex <==
\section{Introduction}
\label{sec:1}
\IEEEPARstart{T}{ensor} is a multidimensional array, which arises naturally in problems where the object is multidimensional and its entries are indexed by continuous or discrete variables. Recovery of tensors under limited sampling and measurements, which is referred to as tensor completion, has been applied to various fields, such as recommendation systems\cite{boumalabsil2011rtrmc}, dimensionality reduction\cite{DBLP:journals/combinatorica/LinialLR95}, multi-class learning\cite{DBLP:journals/sac/ObozinskiTJ10},data mining\cite{4781131,DBLP:conf/sdm/SunPLCLQ09} and computer vision \cite{6138863,Zhang:2014:NMM:2679600.2680311}. In this paper we focus on the tensor completion under the structure of the recently proposed tensor-Singular Value Decomposition(t-SVD), we show that under certain incoherent conditions, one can reconstruct a tensor with low tensor tubal rank with overwhelming probability, given a certain number of samplings.

%Signal recovery from its downsamplings, has been an important research area in statistical signal processing problems related to inversion[cvpr 234] and machine learning for online prediction of ratings[cvpr 5]. The key idea behind such applications is to use the informational complexity of the data itself. For instance, low rank for 2-D matrix, which could also be extended to higher order data via vectorzing the tensor data such as tensor N-rank[cvpr 6]. There are also more general rank related measures of tensors based on HOSVD, Tucker-3 and CP decomposition used in data completion problems[cvpr 7].
In the analysis of multidimensional data, tensor decomposition serves as a useful tool to reveal basic structures if the tensor lies in a low-dimensional space. For example the CANDECOMP/PARAFAC(CP) and Tucker decomposition are two frequently seen decompositions. See \cite{Kolda09tensordecompositions} for a survey of these decompositions. The core idea of the recovery problem based on different decompositions lies on how to create a relationship between the observed entries and the unknown ones. In matrix completion area, which could be regarded as 2nd-order tensor completion, people choose the complexity "rank" of a matrix as a powerful and efficient way to capture certain global information. However, finding the matrix with lowest rank satisfying equality constraints is NP-hard. Candes and Recht\cite{exact_matrix_completion_candes_benj} showed that most low-rank matrices could be recovered from sufficient number of observations by computing the matrix of minimum nuclear norm that agreed with the data matching. Moreover, they gave out the number of samples needed to gaurantee exact recovery with very high probability, given the matrix satisfying the ``incoherent condition". Recht\cite{simpler_approach_benj} developed a much simpler approach to compute the samples needed in the matrix completion problem, which changed the sampling model to sampling with replacement, and used the Noncommutative Bernstein Inequality(NBI). Our work has been greatly inspired by \cite{simpler_approach_benj} and it turns out the NBI is also helpful in our tensor completion problem. We prove that we can perfectly recover a tensor of size $n_1 \times n_2 \times n_3$ with low tensor tubal rank $r$, which we will define later, by simply solving a convex optimization problem, given $O(rn_1n_3 \log(n_2n_3) ) $ samples.

As we will show in the next section, if a third order tensor $\T{X}$ is of CP rank $r$, then its tensor tubal rank is at most $r$. So in this sense it means for any third-order tensor with low CP rank, we can recover it from random samples using this t-SVD structure. Further our technique can be extended to higher-order tensors very easily. Given an $n_1 \times n_2 \times ... \times n_K$ tensor one can reshape it to form a third-order tensor of size $(n_1n_2..n_{k_1}) \times (n_{k_1+1}..n_{K-1}) \times n_K$ and then use our framework for 3-D tensor completion. If $n_k = n$ for all $K$ dimensions then it follows from our main results that $O(n^{\lceil K/2 \rceil} r \log (n^{\lceil K/2 \rceil} )$ measurements are sufficient enough for recovery.

%We note the following points:
%\begin{itemize}
%	\item If a third order tensor $\T{X}$ is of Tucker rank $(r,r,r)$ or CP rank $r$, then its tensor tubal rank is at most $r$.
%	\item Further given an $[n_1,n_2,...,n_K]$ tensor one can reshape it to form a 3-D tensor of size $[n_1n_2..n_{k_1}, n_{k_1+1}..n_{K-1}, n_K]$ be \emph{reshaping} and then use our framework for 3-D tensor completion. If $n_k = n$ for all $k$ then it follows from our main results that ${\cal O}(n^{K/2} r^{K/2-1} n)$ measurements are sufficient enough for recovery.
%\end{itemize}

\subsection{Related Work}
\begin{table*}
	\caption{A summary of existing tensor completion methods}
	\begin{center}
		\begin{tabular}{|p{3cm}|p{4cm}|p{4.5cm}|p{4.5cm}|}
			\hline
			\textbf{Format} & \textbf{Sampling Method} & \textbf{Samples needed for exact recovery (3rd-order tensor of size $n \times n \times n$)}  & \textbf{Incoherent condition} \\ \hline
			CP\cite{DBLP:conf/icml/MuHWG14}  & Gaussian measurements & $O(rn^{2})$ for CP rank $r$ & N/A  \\ \hline
			CP\cite{NIPS2014_5475}  & Random downsample     & $O(n^{3/2}r^5 \log^4(n))$ for CP rank $r$ on symmetric tensors & Incoherent condition of symmetric tensors with orthogonal decomposition \\ \hline
			Tucker\cite{DBLP:conf/icml/MuHWG14} & Gaussian measurements& $O(rn^2)$ for Tucker rank $(r,r,r)$ & N/A \\ \hline
			Tucker\cite{BHuangCmu} & Random downsample & $O(rn^2 \log^2(n))$ for Tucker rank $(r,r,r)$ & Matrix incoherent condition on all mode-$n$ unfoldings \\ \hline
			CP\cite{conf/nips/KrishnamurthyS13} & Adaptive Sampling & $O(nr\log(r))$ for CP rank r & Standard incoherent condition with orthogonal decomposition \\ \hline
			t-SVD(this paper)  & Random downsample & $O(rn^2 \log(n^2))$ for Tensor tubal-rank $r$ & Tensor incoherent condition \\
			\hline
		\end{tabular}
	\end{center}
    \label{table}
\end{table*}

Unlike in the matrix case, the definition of the rank of a tensor is not unique. There are mainly two types of low rank tensor completion, one is based on the CP format, and the other one is based on the Tucker Decomposition. The sampling methods include random downsampling, Gaussian measurements and adaptive sampling. A summary to the best of our knowledge of all the existing methods is concluded in \textbf{Table}~\ref{table}.


\subsubsection{Tensor Completion Based on CP format}
\cite{Karlsson.Kressner.Uschmajew:2014} focused on the tensor completion based on CP format, in which the tensor is represented as a sum of rank-one tensors. Specifically, the CP format of a tensor $\T{X} \in \mathbb{R}^{I_1 \times I_2 \times ... \times I_N}$ of order $N$ is of the following form
\begin{equation}
\label{CP format}
\T{X} = \sum\limits_{\ell=1}^{L} x_\ell^{(1)} \circ x_\ell^{(2)} \circ \dots \circ x_\ell^{(N)},\hspace{2mm} x_\ell^{(n)} \in \mathbb{R}^{I_n}
\end{equation}
where $\circ$ denotes the vector outer product. The smallest $L$ in (\ref{CP format}) is called the CP rank of $\T{X}$. Let $\T{A}$ be the tensor we want to recovery and the set of indices of known entries is $\Omega$. Denote $P_\Omega$ the orthogonal projection onto $\Omega$, \cite{Karlsson.Kressner.Uschmajew:2014} tries to complete the tensor by solving the following optimization problem

\begin{equation}
\min \|P_\Omega(\T{A} - \sum\limits_{\ell=1}^{L} x_\ell^{(1)} \circ x_\ell^{(2)} \circ ... \circ x_\ell^{(N)} ) \|^2_2 + \lambda \sum\limits_{\ell=1}^{L} \sum\limits_{n=1}^{N}\|x_\ell^{(n)}\|_2^2
\end{equation}
where $\lambda \ge 0$ is the regularization parameter. However, this approach has several drawbacks. First, the complexity term here which is the summation of the $\ell_2$ norm of each $x_\ell^{(n)}$ is not a natural choice related to the CP rank and lack of physical explanations. Second, due to the non-convexity of this problem, it only gaurantees local minimum. At end, this method is hard to be used in practical problem since it is difficult to determine the CP rank of a tensor data beforehand, which is regarded as a prior in this approach.

In \cite{NIPS2014_5475} Jain and Oh show that they can recover an $n \times n \times n$ symmetric tensor with CP rank $r$ exactly from $O(n^{3/2}r^5\log^4 n)$ randomly sampled entries. A tensor $\T{X} \in \mathbb{R}^{n \times n \times n}$ is called symmetric in the CP format if its CP decomposition has the format $\T{X} = \sum\limits_{\ell=1}^{r} \sigma_\ell (u_\ell \circ u_\ell \circ u_\ell)$, where $u_\ell \in \mathbb{R}^n$ with $\|u_\ell\| = 1$. They proved that their methods yeild global convergence. Although the authors stressed that their results generalize easily to handle non-symmetric tensors and high-order tensors, there are no theoretical proofs of this.

\subsubsection{Tensor Completion Based on Tucker Decomposition}
Liu et al. \cite{10.1109/TPAMI.2012.39} proposed tensor completion based on minimizing tensor $n$-rank in Tucker Decomposition format, which is the matrix rank of mode-$n$ matricization of a tensor.
Specifically, using the matrix nuclear norm instead of matrix rank, they are trying to solve the convex problem as follows:

\begin{equation}
\begin{aligned}
\label{Tensor n rank}
\min_{\T{X}} &\sum\limits_{i=1}^{n}\alpha_i \|\T{X}_{(i)}\|_*\\
\mbox{subject to  } &P_\Omega(\T{X}) = P_\Omega(\T{T}) 
\end{aligned}
\end{equation}
where $\T{X}_{(i)}$ is the mode-$n$ matricization of $\T{X}$ and $\alpha_n$ are prespecified constants satisfying $\alpha_i \ge 0$ and $\sum_{i=1}^{n} \alpha_i = 1$. It also has several drawbacks. There is no specific way on how to choose weights $\alpha_i$ and normally one just chooses one best matricization according to the results, which turns to a matrix completion problem. It is not applicable to higher-order tensors since no one knows how to assign each $\alpha_i$. Also there is no theoretical guarantees of how many number of samples are required for exact recovery.


There are some modified versions of this problem. \cite{DBLP:conf/nips/Romera-ParedesP13} changed the above complexity term to the convex envelop of cardinality function of singular value vectors, which is proved to be a tighter convex relaxation of the tensor $n$-rank comparing to the above approach. The approach uses the Alternating Direction Method of Multipliers(ADMM) for global convergence guarantees. 

Huang et al.\cite{BHuangCmu} are trying to solve the following strong convex programs, which can be regarded as the combination of the matrix completion and the matrix RPCA, when extended to the case of tensors:

\begin{equation}
\begin{aligned}
\label{tensor n rank 2}
\min_{\T{X},\T{E}} &\sum\limits_{i=1}^{K} \alpha_i \|\T{X}_{(i)}\|_* + \|\T{E}\|_1 +\frac{\tau}{2}\|\T{X}\|^2_F + \frac{\tau}{2} \|\T{E}\|^2_F \\
\mbox{s.t.  } &P_\Omega(\T{X}+\T{E}) = \T{B}  
\end{aligned}
\end{equation}

 They gives out the Tensor Incoherent Conditions(TICs) of exact recovery of tensors using (\ref{tensor n rank 2}) with $\alpha_i = \sqrt{n_i^{(1)}}$, where $n_i^{(1)} = \max \{n_i,\prod_{j \neq i}n_j \}$. It is essentially a direct extension of matrix completion since for each mode-$n$ matricization of the tensor they simply apply the matrix incoherent condition and get a bound for each mode. The number of samples needed for exact recovery also have the same form as matrix completion result. A drawbacks of this approach is that the tensor needs to satisfy the TICS in the unfoldings of every mode, which is impossible to verify in both theory and practice. 

In \cite{DBLP:conf/icml/MuHWG14} Mu et al. are dealing with a different type tensor completion problem. The problem is to complete a tensor with low Tucker rank from Gaussian measurements instead of random downsampling. And certain optimality conditions are given. The core idea is to reshape a multi-dimensional tensor $\T{X} \in \mathbb{R}^{n_1 \times n_2 \times n_3 \times ... \times n_K}$ into a matrix $\T{X}_{(j)} \in \mathbb{R}^{n_1 ... n_j \times n_{j+1}...n_{K}}$ and apply matrix completion on it. It can be shown easily if $\T{X}$ is a low-rank tensor (in either CP or Tucker sense), $\T{X}_{(j)}$ will be a low-rank matrix. They claim if $\T{X}_0$ has CP rank $r$, then $m \ge Crn^{\lceil K/2 \rceil}$ will be sufficient to recover the original tensor. If $\T{X}_0$ has Tucker rank $(r,r,...,r)$, then $m \ge Cr^{\lfloor K/2 \rfloor } n^{\lceil K/2 \rceil }$ is sufficient. 

\subsection{Tensor Completion via Adaptive Sampling}
Krishnamurthy and Singh \cite{conf/nips/KrishnamurthyS13} develop a tensor completion approach based on the adaptive sampling. The key idea is to predict the tensor singular subspace given the sampled subtensor, and recursively update the subspace if a newly sampled subtensor lies out of it. They proved that $O(nr^{3/2}\log r)$ adaptively chosen samples are sufficient for exact recovery when the tensor is of CP rank $r$. And they also concerned a noisy case in their analysis. This approach extends the matrix completion method to the tensor case and yield a tight bound in the area of adaptive sampling.


\subsection{Organization of the paper}
This paper is organized as follows. Section~\ref{sec:2} introduces some notations and preliminaries of tensors, where we defined several algebraic structures of third-order tensors. In Section~\ref{sec:3} we derive the main result on tensor completion and give out the provable bound using t-SVD. We provide the full proof in Section~\ref{sec:4} and we report empirical and numerical results in Secion~\ref{sec:5} . Finally we outline implications of the work and future research in Section~\ref{sec:6}.

